Inducing Social Optimality in Games via Adaptive Incentive Design

How can a social planner adaptively incentivize selfish agents who are learning in a strategic environment to induce a socially optimal outcome in the long run? We propose a two-timescale learning dynamics to answer this question in both atomic and non-atomic games. In our learning dynamics, players adopt a class of learning rules to update their strategies at a faster timescale, while a social planner updates the incentive mechanism at a slower timescale. In particular, the update of the incentive mechanism is based on each player's externality, which is evaluated as the difference between the player's marginal cost and the society's marginal cost in each time step. We show that any fixed point of our learning dynamics corresponds to the optimal incentive mechanism such that the corresponding Nash equilibrium also achieves social optimality. We also provide sufficient conditions for the learning dynamics to converge to a fixed point so that the adaptive incentive mechanism eventually induces a socially optimal outcome. Finally, we demonstrate that the sufficient conditions for convergence are satisfied in a variety of games, including (i) atomic networked quadratic aggregative games, (ii) atomic Cournot competition, and (iii) non-atomic network routing games.

==> extras.tex <==

\subsection{Quadratic Graphon games}
Consider a continuum of players where each agent is indexed by a real number in \([0,1]\). Each player \(x\) chooses a scalar strategy \(s(x)\in \R\). In order to describe the interaction of player \(x,y\in [0,1]\) we define a graphon \([0,1]^2\ni (x,y)\mapsto W(x,y) \in [0,1]\). That is, \(W(x,y)\) measures the level of interaction between players \(x\) and \(y\). Using the Graphon \(W\), the aggregate effect of strategy of neighbors of player \(x\) is defined by 
\[
z(x|s) = \int_{0}^{1} W(x,y)s(y)dy.
\]

In what follows we restrict \(s\in L^{2}([0,1])\). Against the preceding backdrop, we define the cost of player \(x\) under strategy \(s \) as follows:
\[
C(s(x),z(x|s),\alpha(x))
\]
where \(\alpha:[0,1]\ra \R\) characterizes the heterogenity in the utility of different players.

For this game we have 

Observe the similarity with the finite player networked aggregative games. The best response strategy of player \(x\), given all other players play according to the strategy profile  \(s\) is given as follows: 
\[
s_{\br}(x|s) = \arg\max_{\bar{s}} C(\bar{s},z(x|s),\alpha(x)).
\]

A strategy profile \(s_{\ne}\in L^2([0,1])\) with the associated aggregate \(z(\cdot|s_{\ne})\) is a Nash equilibrium if for all \(x\in [0,1]\) we have 
\[
C(s_{\Neq},z(x|s_{\Neq}),\alpha(x)) \leq C(s',z(x|s_{\Neq}),\alpha(x)), \quad \forall \ s'\in \R. 
\]

The social cost of strategy profile \(s\) be given as follows 
\[
S(s) = \frac{1}{2}\int_{0}^1\int_0^1 s(x)Q(x,y)s(y) dxdy + \int_{0}^{1}r(x)s(x)dx 
\]
In order to optimize the social cost we would ideally need the machinery of calculus of variations but we can simplify the objective. 


If we assume that \(Q(x,y)=0\) for all \(x\neq y\) and \(Q(x,x) = q(x)\) then 
\[
S(s) = \int_0^{1}\lr{\frac{1}{2}q(x)(s(x))^2+r(x)s(x)} dx 
\]

Furthermore if \(q(x)>0\) for all \(x\in [0,1]\) then the optimal social allocation is \(\bar{s}(x) = -\frac{r(x)}{q(x)}\). 

Let's work with linear quadratic graphone games. Suppose the cost function of the players is given as follows: 
\begin{align*}
    C(s(x),z(x|s),\alpha(x),\beta(x)) = \frac{1}{2}p(x)s(x)^2 + s(x)\lr{ \alpha(x) z(x|s) + \beta(x)}
\end{align*}
where \(p(x)>0\). The best response strategy profile is: 
\begin{align*}
    s_{\br}(x) = -\frac{1}{p(x)} \lr{ \alpha(x)z(x|s) + \beta(x) }
\end{align*}

Let's assume that the population updates assuming the best response dynamics. 
The update is as follows: 
\begin{align*}
    \frac{d}{dt}s(x,t) &= -\frac{1}{p(x)}\lr{ \alpha(x)\mathbb{W}s(x,t) + \beta(x,t) +p(x)s(x,t)}\\
    \frac{d}{dt}\beta(x,t) = \epsilon \lr{} 
\end{align*}

\subsection{Quadratic Aggregative Game}
Consider a graph \(N\) nodes where each node represents a population of users. Users at each node has to allocate their effort in \(n\) actions. At node \(p\in [N]\), \(x_p^{(i)}\) fraction of players choose action \(i\in[n]\). Let the mass of population \(p\in [N]\) be denoted by \(m_p\).  The cost of population \(p\) on using any effort is affected by neighbor's actions. More formally, the cost incurred by population \(p\) on using action \(i\) is   
\begin{align*}
    C_{p}^{(i)}(x,s) = \frac{m_p^2 q_p^{(i)}\lr{x_p^{(i)}}^2}{2} + x_p^{(i)}\lr{ k_p \sum_{q=1}^{n}G_{pq}x_q^{(i)}} + P_p^{(i)}
\end{align*}
where \(K\in \R^{n\times n}\). More succintly, we can write the cost as follows: 
\begin{align*}
    C_p(x,s) = \frac{1}{2}x_p^\top Q_p x_p + \textsf{diag}(x_p) \lr{ K_p \lr{G_p\kronecker I} x } + P_p
\end{align*}

We consider a perturbed equilibrium 
\begin{align*}
    \perturbEq_p^{(i)}(s) = \frac{\exp(-\eta C_p^{(i)}(\perturbEq(s)))}{\sum_{j=1}^{n}\exp(-\eta C_p^{(j)}(\perturbEq(s)))}, \quad\quad \forall \ i, p
\end{align*}



The social cost of joint effort \(x = (x_1,x_2,...,x_N)\) is  
\begin{align*}
    S(x) = \sum_{p=1}^{N}m_p^2 x_p^\top A_p x_p + m_pB_p^\top x_p.
\end{align*}


\todo[inline]{
Resolve" 
1. Can you justify this social cost? 
}



% \begin{lemma}
% If \(Q+KG\) is invertible, then for any \(p\) Nash equilibrium \(x^\ast(p)\) exists and is unique. 
% \end{lemma}
% \begin{proof}

% Since we are considering the unconstrained setting then for any \(p\), \(x^\ast(p)\) is a Nash equilibrium if and only if \(F(x^\ast(p),p)=0\). That is,  for any \(p\), \(x^\ast(p)\) is the Nash equilibrium if and only if \[
% (Q+KG)x^\ast(p)=-p. 
% \]
% Note that if \(Q+KG\) is invertible then \(x^\ast(p)=-(Q+KG)^{-1}p\) and this is unique.
% \end{proof}

%  Thus the best response strategy update is given by:
% \begin{align}\label{eq: BRDynamics}
%     \dot{x}(t) &= -Q^{-1}\lr{ KGx+p } - x \notag \\ 
%     &= -Q^{-1}\lr{ \lr{Q+KG}x+p}
% \end{align}
% \begin{lemma}
% The best response dynamics \eqref{eq: BRDynamics} will converge if \(\sigma(Q+KG) \subset \C_{+}^{\circ}\). 
% \end{lemma}
% \begin{proof}
% We know that the best response dynamics converges if and only if \(-Q^{-1}(Q+KG)\) is Hurwitz \cite{callier2012linear}. That is \(\sigma(Q^{-1}(Q+KG))\subset \C_{+}^{\circ}\). Since \(Q\) is a positive diagonal matrix the preceding condition holds if and only if  \(\sigma(Q+KG) \subset \C_+^{\circ}\) (refer Lemma 5.4 (3)).  
% \end{proof}


%  Then the pricing dynamics becomes 
% \begin{align*}
%     \dot{\tilde{p}} &= \nabla S(x^\ast(\tilde{p})) \\ 
%     &= Ax^\ast(\tilde{p})+B\\ 
%     &= -A\lr{Q+KG}^{-1}p+B
% \end{align*}


% \subsubsection{Public Good Game}
% Consider a public good game with private provisioning. Let there be \(n\) players, and the income of player \(i\) be denoted by \(m_i\), which is assumed to be fixed. Let agent \(i\in [n]\) provisions \(g_i\) units of public good which is purchased at the price of \(p_i\) per unit of public good. The remaining amount of income is used by agent \(i\) for private consumption \(\pi_i\), which is \(\pi_i=m_i-p_ig_i\). Note that the strategy of every player is the feasible set of public good it can provision. Let \(g=(g_1,g_2,..,g_n) \in \R^n\) denote the vector of all allocations. Using this notation, the total public good provisioned is \(\socGood=\one^\top g\).   


% The utility of player \(i\) depend on the amount used in private consumption and the total social good provisioned. Therefore, the utility of player \(i\) defined by \(u_i(\pi_i,\socGood) = u_i(m_i-p_ig_i,\socGood)\). Furthermore, we make the following assumption about the utility functions: 
% \begin{assm}
% We assume that the private good is \emph{normal}. That is, 
% \begin{align*}
%     -p_i \Der_{12}^{2}u_i(m_i-p_ig_i,\socGood) + \Der_{22}^2 u_i(m_i-p_ig_i,\socGood) \leq 0, \quad \forall g\in \R^n.
% \end{align*}
% \end{assm}


% Given a price profile \(p\in \R^n\), let \(g^\ast(p)\) denote the public goods provisioned by all players in Nash equilibrium. 

% A typical measure of social optimality in this setting is \(S(g) = \sum_{i=1}^{n}h_i(g_i)\), where \(h_i(\cdot)\) is a concave function. Therefore the externality function is 
% \begin{align*}
%     e_i(g^\ast(p),p) &=  \nabla_{g_i}u_i(m_i-p_ig_i^\ast(p), \socGood^\ast(p)) - \nabla h_i(g_i^\ast(p)) \\ 
%     &= \lr{-p_i\Der_1 u_i(m_i-p_ig_i^\ast(p),\socGood^\ast(p)) + \Der_2 u_i(m_i-p_ig_i^\ast(p),\socGood^\ast(p))} - \nabla h_i(g_i^\ast(p))
% \end{align*}

% Computing the conditions stated in Proposition \ref{prop: ConvergenceTildeP}. We compute \(\frac{\partial e_i(g^\ast(p),p)}{\partial p_j}\) below: 
% \begin{align*}
% &\frac{\partial e_i(g^\ast(p),p)}{\partial p_j} = {\color{blue}\frac{\partial \socGood^\ast(p)}{\partial p_j}} {\color{red}\lr{-p_i \Der_{12}^2u_i(m_i-p_ig_i^\ast(p),\socGood^\ast(p)) + \Der_{22}^2u_i(m_i-p_ig_i^\ast(p),\socGood^\ast(p))  }} \\ 
% &+{\color{brown}\frac{\partial g_i^\ast(p)}{\partial p_j}}\lr{{\color{cyan}  p_i^2 \Der_{11}^2  u_i(m_i-p_ig_i^\ast(p),\socGood^\ast(p)) -p_i \Der_{21}^2 u_i(m_i-p_ig_i^\ast(p), \socGood^\ast(p))  }- {\color{gray} \nabla^2h_i(g_i^\ast(p))}}
% \end{align*}

% We expect the {\color{blue}blue} term to be negative and {\color{red}red} term is negative by normality assumption on the private good. From Proposition 2 in Daron's paper we can ensure that {\color{brown}brown} term is positive and {\color{cyan}cyan} is negative. Furthermore, the {\color{gray}gray} term is negative from the concavity of \(h\). This is where there is conflict between the cyan terms and the gray term. 
% \todo[inline]{Notes: 

% I think the current setting for public good games is not directly amenable to our analysis. This is because the strategy set is dependent on the price and thus the variational inequalities for social cost and Nash equilibrium cannot be matched.
% }

% Example include 
% \(u_i(m_i-p_ig_i,G)= \ln(m_i-p_ig_i) + \alpha_i \ln(G) \). Constraints are \(m_i \geq p_i g_i\). 
